Query Augmentation by Decoding Semantics from Brain Signals

Query augmentation is a crucial technique for refining semantically imprecise queries. Traditionally, query augmentation relies on extracting information from initially retrieved, potentially relevant documents. If the quality of the initially retrieved documents is low, then the effectiveness of query augmentation would be limited as well. We propose Brain-Aug, which enhances a query by incorporating semantic information decoded from brain signals. BrainAug generates the continuation of the original query with a prompt constructed with brain signal information and a ranking-oriented inference approach. Experimental results on fMRI (functional magnetic resonance imaging) datasets show that Brain-Aug produces semantically more accurate queries, leading to improved document ranking performance. Such improvement brought by brain signals is particularly notable for ambiguous queries.

==> latex/abstract_old.tex <==

% Ziyi has finished the abstract
% Understanding users' information needs is crucial for improving search performance. 
% Since queries submitted by the user are often imprecise, vague, or inaccurately phrased, the query augmentation technique is adopted to refine semantically imprecise queries.
Query augmentation is a crucial technique for refining semantically imprecise queries.
Traditionally, query augmentation relies on extracting information from potentially relevant documents.
For example, existing work has adopted explicit web interaction contexts, such as clicks and dwelling time, to learn user context for augmentation.
However, explicit interactions are not always available and only function as a probe for the user's thoughts.
With the recent advances in portable neurophysiological devices, existing studies have successfully improved ranking performance by reformulating the query with contents extracted from documents that are inferred as relevant with the help of brain signals.

However, existing studies rely on interactions between users and the retrieved documents. 
Query reformulation without prior interactions with document contents is an open problem.
To address this, we propose Brain-Aug, a query augmentation method that decodes semantic information from brain signals. 
Brain-Aug employs brain signals to generate the continuation of the original query for query augmentation with a prompt tunning training protocol and a ranking-orient inference approach. 
Experimental results on fMRI datasets show that Brain-Aug can reformulate queries based on users' mental activities, leading to improved document ranking performance. 
Further analysis shows that the improvement brought by brain signals is particularly notable for ambiguous queries.


==> tables/case_study2.tex <==
\newlength{\dlength}
% 设置长度 x 的值为 3cm
\setlength{\dlength}{3.3cm}
\begin{table} % 使用figure环境包裹表格以便添加标题和标签
\caption{\textcolor{blue}{Example of IRF and RRF results for participant ID 1 and query ``The Prophet'' with task description ``explore the concepts of prophet in the general domain''. Documents with relevance annotations of 4 and 2-3 are highlighted in \textcolor{myPurple}{purple} and \textcolor{myLightPurple}{light purple}, respectively. Documents with annotations of 1 are presented in \textcolor{black}{black}.}}
  \centering % 居中对齐
  \begin{minipage}{0.5\linewidth} % 使用minipage环境将三个表格并排放置，每个占总宽度的1/3
    \centering
    \subcaption{\textcolor{blue}{The titles~(translated into English) for historical documents~($D^h$) and unseen documents~($D^u$).}}
    \label{tab:split_table1}
    \input{tois2023ye/meta/split_table1}
  \end{minipage}
  \hfill % 添加水平空白，以使表格之间平均分布
  \begin{minipage}{0.45\linewidth}
    \begin{minipage}{\linewidth}
        \centering
        \subcaption{\textcolor{blue}{The estimated base relevance scores for historical document $D^h$, $R^c$, $R^p$, and $R^bs$ represent click-based, pseudo-relevance based, and brain-based scores, respectively.}}
        \label{tab:split_table2}
        \input{tois2023ye/meta/split_table2}
    \end{minipage}
    \vspace{1cm}
    \vfill
    \begin{minipage}{\linewidth}
        \centering
        \subcaption{\textcolor{blue}{The re-ranked documents list for IRF \& RRF tasks across RF models with and without brain signals~(w $R^{bs}$ and w/o $R^{bs}$).}}
        \label{tab:split_table3}
        \input{tois2023ye/meta/split_table3} 
    \end{minipage}
  \end{minipage}
\end{table}





